Fractional models of Reynolds-averaged Navier-Stokes equations for Turbulent flows

Its is a well known fact that Turbulence exhibits non-locality, however, modeling has largely received local treatment following the work of Prandl over mixing-length model. Thus, in this article we report our findings by formulating a non-local closure model for Reynolds-averaged Navier-Stokes (RANS) equation using Fractional Calculus. Two model formulations are studied, namely one- and two-sided for Channel, Pipe and Couette flow, where the results shown have less 1% error. The motivation of two-sided model lies in recognising the fact that non-locality at a given spatial location is an aggregate of all directions. Furthermore, scaling laws and asymptotic relationship for Couette, Channel and Pipe flow is reported. It is to be noted that modeling in wall units, no additional coefficient appears, thus there models could be applied to complex flows with ease.

==> hist.tex <==
\section{Fractional Integral, Derivative and Laplacian } \label{lap}


Leibniz introduced the notation ($d^n / dy^n$) for $n^{th}$ order differentiation. This prompted L'hospital to ask for the differentiation with $n = 1/2$, replying to his letters in 1695, Leibniz mentioned it as an apparent paradox for which one day will have use full consequences. This conversation is the earliest record of Fractional derivative. A brief history about its origins is detailed in chapter 1 of \cite{Ross1975}. The first appearance of the mathematical form as generally accepted today's definition of Fractional integral is given Abel's integral equation \cite{Abel1826, abel_2} as given in section 2.1 of \cite{samko1993fractional} with the Euler function ($ \Gamma$) used for convenience. 

\begin{equation}
    f(x) =  { 1 \over \Gamma(\alpha)  } \int_{0}^{x} {\psi(t) dt  \over { (x -t)^{\alpha}   }} 
\end{equation}

However, Abel himself did not solve the equation for $\alpha = 1/2$ in the spirit of Fractional integration. The modern notation of fractional integro-differentiation were established during his time. The significance of this definition is the fractional integral of order ($1 -\alpha$) as given by Riemann \cite{riemann_2013}, while the inversion of this definition is the fractional differentiation \cite{samko1993fractional}. 

==> methodology.tex <==
\section{Numerical Methodology} \label{methodology}
%
%
% Numerical methodology 
%
% 1. Fractional derivative discretisation
% 2. PINNs outline


